Enhancing Maritime Situational Awareness through End-to-End Onboard Raw Data Analysis

Satellite-based onboard data processing is crucial for time-sensitive applications requiring timely and efficient rapid response. Advances in edge artificial intelligence are shifting computational power from ground-based centers to on-orbit platforms, transforming the "sensing-communication-decision-feedback" cycle and reducing latency from acquisition to delivery. The current research presents a framework addressing the strict bandwidth, energy, and latency constraints of small satellites, focusing on maritime monitoring. The study contributes three main innovations. Firstly, it investigates the application of deep learning techniques for direct ship detection and classification from raw satellite imagery. By simplifying the onboard processing chain, our approach facilitates direct analyses without requiring computationally intensive steps such as calibration and ortho-rectification. Secondly, to address the scarcity of raw satellite data, we introduce two novel datasets, VDS2Raw and VDV2Raw, which are derived from raw data from Sentinel-2 and Vegetation and Environment Monitoring New Micro Satellite (VENuS) missions, respectively, and enriched with Automatic Identification System (AIS) records. Thirdly, we characterize the tasks' optimal single and multiple spectral band combinations through statistical and feature-based analyses validated on both datasets. In sum, we demonstrate the feasibility of the proposed method through a proof-of-concept on CubeSat-like hardware, confirming the models' potential for operational satellite-based maritime monitoring.

==> sections/07_reference.tex <==
\newpage

{\footnotesize
 	\begin{spacing}{1.6}% tune the size by altering the parameter
 		\bibliography{bibliography} % Include your own bibliography (*.bib), style is given in isprs.cls
 	\end{spacing}
 }
 

==> sections/in_cursus/SIoU.tex <==
The \textbf{Scale-adaptive Intersection over Union (SIoU)} is a novel similarity metric specifically designed to address the limitations of the traditional Intersection over Union (IoU) in small object detection tasks. Traditional IoU is scale-invariant, meaning it does not change when the bounding boxes are uniformly scaled. While this property may seem advantageous, it actually causes IoU to be overly sensitive to small localization errors, particularly when detecting small objects. To mitigate this issue, SIoU introduces a scaling factor \( p \) that adapts according to the size of the objects, making the metric more lenient towards small shifts in smaller objects.

The mathematical formulation of SIoU is as follows:

\begin{equation}
\text{SIoU}(b_1, b_2) = \text{IoU}(b_1, b_2)^p
\end{equation}

Where the scaling factor \( p \) is defined by:

\begin{equation}
p = 1 - \gamma \exp\left(-\frac{\sqrt{w_1h_1 + w_2h_2}}{\sqrt{2\kappa}}\right)
\end{equation}

Here:
\begin{itemize}
    \item \( b_1 \) and \( b_2 \) are the two bounding boxes being compared, with dimensions \( w_1, h_1 \) and \( w_2, h_2 \) respectively.
    \item \( \gamma \) is a parameter that controls the degree of scaling, particularly for smaller objects.
    \item \( \kappa \) is a parameter that influences how quickly the scaling effect diminishes as the object size increases.
    \item \( \exp \) denotes the exponential function, which ensures that the scaling factor \( p \) diminishes gradually, depending on the size of the bounding boxes.
\end{itemize}

This formulation allows SIoU to be more forgiving of small inaccuracies in bounding box localization for smaller objects, thus providing a more robust and perceptually aligned measure of object detection performance. Consequently, SIoU is especially useful in contexts such as Few-Shot Object Detection (FSOD), where the ability to accurately detect small objects despite limited data is crucial.

==> sections/in_cursus/stripe.tex <==
Multi-spectral images are unavoidably contaminated by various types of impulse noises such as salt and pepper noise, missing pixels, missing lines and other outliers. 



The signal-to-noise ratio (SNR) is usually estimated as the ratio of the signal electrons generated by the photons flux and the square root of the number of noise.



In remote sensing images, the stripe effects can be regarded as additive noise, and the degradation model can be given by:
\begin{equation}
f(x, y) = u(x, y) + s(x, y) + n(x, y)
\end{equation}

where for $x = 1, 2, \cdots, M$, $y = 1, 2, \cdots, N$, $M$ and $N$ denote the number of rows and columns of the 2-D gray-level image, respectively. Here, $f(x, y)$, $u(x, y)$, $s(x, y)$, and $n(x, y)$ stand for the pixel values of the observed image, the ground-truth image, the additive stripe component, and the Gaussian white noise at the location $(x, y)$, respectively.

Instead of the formulation of \cite{chen2017stripe}, we model the noise term using the formulation of \cite{longepe2024simulation}.
Therefore, our noise term considers 
signal degradation due to (a) Signal-to-Noise Ratio (SNR) and (b) Module Transfer Function (MTF). This approach leads to a more realistic simulation of the noise affecting raw multi-spectral images.


The term for signal degradation due to SNR is constructed as:

\begin{equation}
N(i, j) = \frac{DN_{ref}}{SNR} \cdot \mathcal{N}(0, 1)
\end{equation}



PSF:
Step that simulates loss of signal due to limited bandwidth of the Module Transfer Function (MTF), which is equivalent to simulate the Point Spread Function (PSF) for the entire system (imager and platform).

is not too extended, approximating the optical PSF as independent of the position inside the field of view is reasonable. This approximation allows the optical system to be considered shift-invariant with a well-defined transfer function, and the blurring effect can be modeled as a convolution between the PSF and the scene intensity

The MTF filter is two-dimensional with independent across- and along-track parameterization

==> v0/SRC.tex <==
% The selected region of interest (ROI) for this work is the open sea in front of the port of Ashdod in Israel. The VENµS MSI captured the ROI at around 8:30 UTC every two days during the first scientific mission phase.
% The AIS data for vessels within the ROI was retrieved from the maritime analytics provider MarineTraffic\footnote{www.marinetraffic.com}. 
% However, the dataset has a limitation: it only provides one AIS record per vessel per day within the ROI during the 3-year fist mission phase, typically around midnight UTC. This means that information about a vessel's position, when the spacecraft sensed the ROI, is unavailable.
% On the other hand, most vessels spend extended periods (i.e., several days) stationary, waiting for port authority authorization to enter the port. This standard procedure allows port authorities to schedule traffic based on the ships' characteristics and current conditions \cite{Ma2023}.
% The database includes 3,827 vessels with bounding box labels in 282 multispectral images captured during the VENµS VM01 mission phase. Among these vessels, 2,733 (71.4\%) have corresponding Automatic Identification System (AIS) records in the MarineTraffic database. The AIS database identifies 18 different vessel types. Table \ref{fig:venus_ais} shows statistics on the length and width of vessels for each type in the AIS database.
%
% \begin{table}[h!]
%     \renewcommand{\arraystretch}{1.2}
%     \caption{Summary Statistics of Vessels Dimension by Type.}
%     \label{table:VENuS_bbox}
%     \centering
%     \begin{tabular}{*8c}
%         \hline 
%         Vessel Type  & Count & Mean Length & Max. Length & Min. Length & Mean Width & Max. Width & Min. Width \\
%         \hline 
%         General Cargo                       &  1637 &  105.13 &  199.99 & 69.10 & 16.28 & 28.60 & 9.95 \\
%         Bulk Carrier                        &  554  &  168.84 &  234.98 & 112.80& 26.80 & 38.00 & 16.80 \\
%         Container Ship                      &  323  &  175.56 &  368.00 & 92.80 & 25.86 & 51.00 & 16.20 \\
%         Oil/Chemical Tanker                 &  112  &  116.65 &  195.00 & 64.60 & 18.98 & 32.29 & 15.20 \\
%         Cement Carrier                      &  40   &  91.44  &  96.63  & 80.00 & 15.23 & 16.01 & 13.60 \\
%         Cargo/Containership                 &  30   &  109.36 &  132.23 & 89.78 & 17.08 & 20.20 & 13.60 \\
%         Tanker                              &  12   &  182.58 &  183.00 & 89.78 & 29.67 & 32.00 & 13.60 \\
%         Heavy Load Carrier                  &  5    &  143.52 &  228.12 & 111.60& 23.98 & 43.00 & 16.80 \\
%         Vehicles Carrier                    &  4    &  179.52 &  183.28 & 176.00& 31.49 & 32.25 & 31.10 \\
%         Cargo                               &  3    &  130.76 &  130.76 & 130.76& 17.70 & 17.70 & 17.70 \\
%         Oil Products Tanker                 &  3    &  151.99 &  179.99 & 96.00 & 26.47 & 32.20 & 15.00 \\
%         Tanker - Hazard A (Major)           &  3    &  182.00 &  182.00 & 182.00& 32.00 & 32.00 & 32.00 \\
%         Tanker - Hazard D (Recognizable)    &  2    &  175.50 &  180.00 & 171.00& 30.00 & 32.00 & 28.00 \\
%         Drill Ship                          &  1    &  228.00 &  228.00 & 228.00& 42.00 & 42.00 & 42.00 \\
%         Offshore Supply Ship                &  1    &  78.25  &  78.25  & 78.25 & 17.20 & 17.20 & 17.20 \\
%         Reefer                              &  1    &  144.52 &  144.52 & 144.52& 21.80 & 21.80 & 21.80 \\
%         Tanker - Hazard C (Minor)           &  1    &  176.00 &  176.00 & 176.00& 31.00 & 31.00 & 31.00 \\
%         Other                               &  1    &  72.00  &  72.00  & 72.00 & 22.00 & 22.00 & 22.00 \\
%         \hline 
%     \end{tabular}
% \end{table}



Table \ref{table:STD} presents the standard deviation (STD) values calculated for each spectral band of VEN$\mu$S L0 and L2 images captured over a cloud-free open sea area, spanning approximately 11 square kilometres and devoid of any vessels or other objects. The image acquisition date is May 14th, 2018. Figure \ref{fig:STD} depicts the normalized STD across the 12 bands for both L0 and L2 images. Standard deviation quantifies the variability in pixel values, with higher STD values indicating increased noise levels. Additionally, normalized STD values have been derived.
Generally, the standard deviation in L0 images surpasses the corresponding L2 images across all bands, indicating a denser value distribution in the L2 images.
The comparison between L0 and L2 images is essential, considering that L2 is the standard product commonly employed for EO analysis despite inherently possessing higher noise levels than L0 images, which are more conducive for scientific purposes.
Figures \ref{fig:L0_examples} (c) and (d) display the VENµS L0 and L2 images, respectively, over various agricultural fields. The L0 image, while not georeferenced, also exhibits geometric distortions due to sensor tilt and topographic variations. The L2 image is ortho-rectified at a ground resolution of 5 m on a UTM projection.


- We have to show that we need more than a single band for achieving good results.

- We want to show the results on two diverse dataset to demonstrate the generalizations and applicability of our method to different sensors and different areas.

- We want to show the difference in with and coarse and fine coregsitration technique, accepting a small value of diff.

Show the results on the two datasets for:
\subsection{Coarse and fine coregistration}
\hl{@Manuel, Gabriele} \\
\hl{- Trying to quantify the mean average coregistration error on the datasets.}

In line with our previous discussion, optimizing the onboard co-registration process was not the main focus of this study. We evaluated the performance of two co-registration solutions for the 12 bands of the VENµS multispectral camera. The analysis was conducted using cloud-free data from 14th May 2018, which included 22 vessels detected on the open sea within the L0 image. For each vessel, we manually computed the shift in both horizontal (X) and vertical (Y) directions between all VENµS bands and band 5 (reference band). Table \ref{table:error_coreg} summarizes the average shift values in the X and Y directions for the 22 vessels, categorized by coarse and fine co-registration. The table also includes the detector associated with each band. As a reminder, band 5 is the first band acquired by detector A of the VSSC (see Figure \ref{fig:VSSC_detector}).

The results demonstrate a clear correlation between the coarse co-registration performance and the detector location. Bands acquired with the same detector as band 5 (detector A) exhibited the smallest X-direction shift, averaging 0.64 pixels. Bands from the subsequent detector B (bands 10-12) displayed the second-best performance in the X-direction, with an average displacement of approximately 4.2 pixels. The largest X-direction displacements were observed for bands associated with detector D (bands 3, 4, and 6), averaging around 10 pixels.

==> v0/intro_old.tex <==
\section{Introduction}\label{INTRODUCTION}

Considering the enormous impact on civil maritime applications, the efficient and timely detection of vessels using Earth Observation (EO) satellite imagery is imperative for scenarios requiring rapid response, such as maritime surveillance, environmental monitoring, and emergency search and rescue operations. Traditional data processing chains based on the classical bent-pipe approaches \cite{furano2020towards,GiuffridaPhiSat} pose significant challenges in addressing these needs effectively due to several inherent limitations, such as the increased latency for data download, 
ground station availability and high-level product calculation. 
Indeed, high latency response is a crucial issue with the current data handling chain, which involves the transmission of vast quantities of raw satellite data to ground-based processing facilities. This data transmission and subsequent processing incur substantial delays from image acquisition to the delivery of actionable information \cite{meoni2024unlocking}. Such delays are critical impediments in scenarios that demand immediate action, such as detecting and responding to illegal fishing activities or maritime accidents.
Additionally, the need to transmit data from satellites to Earth strains the available communication bandwidth \cite{furano2020towards,GiuffridaPhiSat}. 
% This constraint is particularly pronounced for high-resolution satellites and can limit the frequency and resolution of satellite passes, thus affecting the timeliness and quality of the data received.
\newline
To mitigate these issues, numerous works have explored the use of Artificial Intelligence (AI) on board satellites for fast retrieval of actionable information for latency-constrained applications, such as natural disasters \cite{mateo-garcia_towards_2021,diana2021oil,meoni2024unlocking,del2021board}, or fast retrieval of actionable information, such as changes or targets in local areas \cite{ruzicka2022ravaen}. 
%
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/general_description.png}
%     \caption{Graph comparing the traditional data handling chain with the onboard AI approach. The onboard AI approach significantly reduces latency by bypassing many power demanding ground processing steps, and delivering the information directly to the end user.}
%     \label{fig:aionboard}
% \end{figure}
% -- TO BE ADDED SOMETHING RELATED TO HIGH-END DATA-- TALK ABOUT RAW DATA
% Satellites, especially smaller classes like micro and nanosatellites, are equipped with limited computational resources. This limitation restricts the complexity of the data processing tasks that can be performed onboard, thereby necessitating reliance on ground-based processing. Moreover, onboard data processing, while beneficial for reducing latency, significantly increases the energy demands on the satellite. This increased consumption can impact other critical satellite functions and shorten the mission lifespan due to the finite energy resources available on most satellites. 
% \newline
%Despite these challenges, the recent advancements in edge computing with Artificial Intelligence (AI) led to unprecedented benefits in terms of computational efficiency and inference times, opening a new space sector. 
This motivated the recent launch of $\Phi$Sat-2 from the European Space Agency (ESA), Intuition-1 from KP Labs, CogniSAT-6U from Ubotica, and Kanyini\footnote{https://smartsatcrc.com/research-programs/kanyini-sa-space-services-mission/}, a new generation of satellites embarking AI-enabled chips. 
\newline
The present manuscript configure itself in this framework, detailing the onboard application of AI for improving Maritime Domain Awareness (MDA).
%
% \paragraph{Background}\label{sec:backg}
% With approximately 70\% of the Earth’s surface covered by oceans, the importance of conserving and sustainably utilizing marine resources cannot be overstated. Oceans play a pivotal role in regulating the global climate, supporting biodiversity, and providing livelihoods for millions of people. As outlined by the United Nations (UN)\footnote{https://sdgs.un.org/goals/goal14}, sustainable development necessitates the careful management of these vital ecosystems to ensure their health and productivity for future generations. Effective strategies for the conservation and sustainable use of oceans and seas involve reducing pollution, protecting marine habitats, and promoting responsible fishing practices. 
% \newline
% For these reasons, acquiring knowledge of human activities at sea has always been a crucial issue for the remote sensing community.
% In the past, maritime monitoring services based on the Automatic Identification System (AIS) were used to measure marine traffic. 
% Notwithstanding, the International Maritime Organization (IMO) \cite{balkin2006international}, regulates that only certain classes of vessels must embark an AIS transmitter, i.e., medium and large ships ($>$ 300 tons). It must be noted that the AIS transmitter can be deliberately turned off or masked, rendering the AIS data incomplete or inaccurate. As a result, AIS information alone is insufficient for comprehensive maritime monitoring, as it is estimated that up to 75\% of commercial marine traffic operates without it \cite{paolo2024satellite}. 
% Therefore, although AIS provides valuable data on the identification and route information of medium and large vessels, its limitations necessitate the integration of additional data sources for effective maritime surveillance. It is essential to incorporate supplementary data from other remote sensing technologies to address these gaps. Synthetic Aperture Radar (SAR) and optical imagery have demonstrated their utility in enhancing MDA.
% While most of the research for vessel detection focused on SAR data \cite{eldhuset1996automatic}, \cite{tello2006automatic}, and \cite{zhang2019ship}, optical imagery represents a complementary data source. 
Past methodologies for optical data employed disparate approaches into absolving the task of vessel recognition. Without loss of generality, we can distinguish the methods into: a) Threshold Segmentation Methods, b) Statistical Methods, c) Feature-Based Methods, and d) Deep-Learning Methods.
\newline
    Threshold-based methods aim to differentiate ships from the background by analyzing the differences in reflectance values. This technique relies on identifying distinct gray value thresholds to segment the image, effectively separating the ships from the surrounding environment. Notable works in this area include studies by \cite{burgess1993automatic}, \cite{corbane2008using} and \cite{heiselberg_direct_2016}. 
    % Notably, \hl{Yao et al. (2018)} implemented a local saliency map approach with fixed thresholds, while the proposed chain’s adaptive thresholding proved more effective.
\newline
    Statistical methods focus on analyzing the gray value distributions within ship scenes. By examining the statistical properties of these gray values, these methods can identify and distinguish ships from the background. Key contributions to this approach have been made by \cite{proia2009characterization} and \cite{yang_ship_2014}, as well as Corbane et al. in their various studies \cite{corbane2008fully} and \cite{corbane2010complete}.
\newline
    Feature-based methods place significant emphasis on the features derived from traditional image processing techniques. By extracting and analyzing the feature descriptors, these methods can effectively identify ships. The work of \cite{zhenwei_shi_ship_2014} has made substantial contributions to the development of feature-based methods, addressing the ship detection in high-resolution optical panchromatic imagery, proposing a hierarchical detector employing Histogram of Oriented Gradients (HOGs) \cite{dalal2005histograms}. The work of 
    \cite{guo2012novel} employs instead the SIFT (Scale Invariant Feature Transform) \cite{lowe2004distinctive} features.
\newline
    Deep-Learning methods utilize learned weights to produce a latent representation of a vessel by training models on large datasets. Zhu et al. have made notable advancements in applying deep learning techniques for vessel detection. Recently, the work of \cite{ciocarlan_ship_2021} employed a Self-Supervised Learning (SSL) approach for the segmentation of vessels in Sentinel-2 images. The work demonstrates that SSL is more effective in frugal conditions than training from scratch or using transfer learning from other domain datasets, e.g., ImageNet. The study of \cite{mayra4827287mapping} uses Sentinel-2 imagery and the YOLOv8 object detection framework to identify and quantify small vessels in Finnish marine areas. The analysis, covering five locations, involved annotating 7,807 vessels. The best models achieved high accuracy.
\newline
    Threshold methods suffer from a lack of generality and need manual tuning to deal with different kinds of scenarios but are easy to implement and highly scalable. Statistical methods performance depends on the selected statistical model for describing the sea surface clutter, which can be different at inference time, therefore performing poorly on medium-resolution multi-spectral imagery.
    Feature-based methods are mature in engineering but 
\newline
    DL methods have been lately developed with the insurgence of greatly improved computing capabilities led by Graphic Computation Units (GPUs). They show great generalizability and can benefit from the recent push towards space-graded AI devices in space \cite{meoni2024unlocking}. They stand unrivaled in terms of performance but they require labelled datasets to learn the inherent patterns and data distribution in order to solve a downstream task.
\newline
% CLASSIFICATION:
Ship-type classification is not only a crucial aspect of maritime surveillance but also challenging, as noted by \cite{heiselberg_direct_2016}. In Sentinel-2 images, supervised classification can roughly identify ship types (e.g., \textit{Cargo}, \textit{Tankers}) with accuracy that depends on image resolution. Owing to the 10m resolution bands, this results in a lack of features necessary for precise identification, such as meter-level precision measurements, exact contours, or distinct traits. 
For these reasons, \cite{heiselberg_direct_2016} states that classification is doable only when vessels are longer than 30m.
\newline
Research in this domain can be broadly categorized based on the type of data utilized (e.g., AIS data and imagery data) and, additionally, the classification can be approached from either a coarse-grained or fine-grained level \cite{liu2017high,9044734}.
AIS data benefits from being less affected by weather conditions and utilizing both static information (e.g., Maritime Mobile Service Identities (MMSI), dimensions, ship-type) and dynamic information (e.g., position, speed) and can be used to develop algorithms and models to classify ships based on their attributes. Various techniques have been applied to AIS data and demonstrate high accuracy rates, including partitioning techniques \cite{zhou2019ship}, Graph Neural Networks \cite{li2021ship}, Convolutional Neural Networks (CNNs) \cite{yang2022ship}, logistic regression models \cite{sheng2018research}, and integration with other sources \cite{yan2022ship}.
%These methods have shown high accuracy rates, demonstrating the effectiveness of machine learning in addressing challenges like missing or tampered ship-type information in AIS data. Researchers have also explored integrating AIS data with other sources such as satellite imagery and radar data to enhance classification accuracy and reliability (Wang et al., 2020; Yan et al., 2021)
On the other hand, advanced image processing techniques, including machine learning and computer vision, enable the extraction of meaningful features from images, facilitating accurate ship classification tasks. Image data is particularly useful in scenarios where visual verification is required or where AIS data might be incomplete or tampered with \cite{9216603}. \hl{magari espandere un po' qui, aggiungendo altre ref}% other ref qui
\newline
When considering the distinction between coarse- and fine-grained classification, ships are divided into broad categories based on specific criteria, i.e., general categories \cite{joseph2019novel} or moving ships and static ships \cite{8412136}, and labelled by their precise type \cite{9044734}, respectively. Coarse-grained methods typically compare extracted ship features with a priori information, while fine-grained methods often employ CNNs to identify ship types accurately. Additionally, a significant challenge in ship classification is the lack of a universally accepted standard for data annotations, which can affect the consistency and accuracy of classification efforts.
\newline
Many studies in the literature utilize images with a spatial resolution exceeding 4m for coarse-grained classification methods \cite{gallego2018automatic,joseph2019novel,8405523}. In comparison, fine-grained classification methods are typically applied to images with a spatial resolution greater than 2m \cite{9044734,luu2019improving,7911301}. \cite{8902822} conducts classification using Sentinel-2 images with a 10m spatial resolution. \hl{aggiustare cites}

\paragraph{Overview of onboard processing with ML}\label{sec:problem-statement}
Assigned to \hl{@Gabriele: TOBECOMPLETED}

% \paragraph{Motivation of the work}\label{sec:problem-statement}
Given these challenges and opportunities, there is the possibility to develop advanced processing methodologies and datasets that would allow processing directly on board satellites. As mentioned, such methodologies would minimize data transmission, reduce latency, and optimize the use of limited satellite resources, thereby enhancing the capability of satellite systems to provide near-real-time, actionable data for critical maritime operations. 
On the other hand, the datasets enable the capture of the inherent data distributions of raw data, which is necessary to train proper models.
\newline
This paper addresses both issues by implementing a lightweight, energy-efficient pre-processing strategy cascaded to a DL technique for direct vessel identification. Extensive tests are calculated on raw satellite imagery from Sentinel-2 and VENµS.
%
% \paragraph{Novelties of the work}\label{sec:problem-statement}
In summary, this research introduces several novel contributions. Firstly, it represents the pioneering implementation of a fully integrated end-to-end workflow tailored for onboard vessel detection. Streamlining the entire process from data acquisition to detection significantly reduces latency and enhances the efficiency of maritime surveillance operations. Secondly, this work is the first to leverage raw, uncalibrated satellite data for end-to-end maritime vessel detection. Utilizing directly raw data, we enhance the real-time processing capabilities of the next generation of small satellites. To deal with this unused data distribution, we provide the scientific community with two comprehensive datasets for vessel detection and classification. Lastly, the research demonstrates an optimized model deployment for dealing with the limited computational resources available onboard. These innovations collectively push the boundaries of current satellite data processing methodologies, enabling more timely and accurate detection of vessels, which is crucial for a range of maritime applications.
\newline
The contributions of the manuscript in this research are multifaceted but can be grouped as follows. 
The first two datasets of raw, uncalibrated multi-spectral data for vessel detection and classification have been generated from scratch using Sentinel-2 and VENµS missions. These datasets have been compiled using additional AIS information, further reinforcing the representativeness of the data. Additionally, we propose a novel format for storing annotations, comprehensive of both bounding boxes and AIS records.
These pioneering datasets serve as a foundational resource, offering diverse and unprocessed scenarios essential for the development and validation of detection algorithms.
Based on these datasets, as previously demonstrated in \cite{meoni2023thraws} for wildfires, we demonstrate that the coarse coregistration technique can also be applied for the task of vessel detection and classification. In this methodology, spectral bands are registered together based on pre-determined look-up tables. 
Applying DL-based techniques to the developed datasets, we demonstrate which are the most useful bands for practising detection or classification.
We correlate these results with additional information about the spectral bands. Through the analysis of different geographic areas with different sensors and resolutions, we show very comparable results, further reinforcing the generalizability of our approach dealing with raw data. 
Finally, an onboard implementation is presented, showcasing a proof-of-concept realised on space-graded AI edge-device. 
\newline
% \paragraph{Final Statement}\label{sec:problem-statement}
The remainder of the paper is structured as follows: Section 2 details the data creation and curation strategy of the first two raw multispectral datasets for vessel detection and classification enriched with AIS information. 
Section 3 discusses the proposed methodology of the cascaded application of coarse coregistration and DL-based detection.
Section 4 reports the results on the developed datasets demonstrating the generalization and applicability of the proposed technique.
Section 5 is devoted to the onboard implementation to demonstrate a proof-of-concept.
Finally, Section 6 concludes the paper.

